ToolGrad: Efficient Tool-use Dataset Generation with Textual "Gradients"

Prior work synthesizes tool-use LLM datasets by first generating a user query, followed by complex tool-use annotations like depth-first search (DFS). This leads to inevitable annotation failures and low efficiency in data generation. We introduce ToolGrad, an agentic framework that inverts this paradigm. ToolGrad first constructs valid tool-use chains through an iterative process guided by textual "gradients", and then synthesizes corresponding user queries. This "answer-first" approach led to ToolGrad-500, a dataset generated with more complex tool use, lower cost, and almost 100% pass rate. Experiments show that ToolGrad models outperform those trained on expensive baseline datasets and proprietary LLMs. The ToolGrad source code, dataset, and models are available at https://github.com/zhongyi-zhou/toolgrad.

==> contents/00_teaser.tex <==
\makeatletter
\AtBeginDocument{
\let\@oldmaketitle\@maketitle
\renewcommand{\@maketitle}{\@oldmaketitle
  \includegraphics[width=\linewidth]{figures/Teaser-landscape-v6.pdf}
  \captionof{figure}{Prior art for tool-use dataset generation (top) starts with a user query, followed by an expensive, failure-prone tool search (\eg, DFS). In contrast, \systemname (bottom) first generates successful tool-use chains, then annotates corresponding user queries, achieving superior efficiency and almost 100\% pass rate. 
  }
  \label{fig:teaser}
 }
}
\makeatother







